A method for bounding high-order finite element functions: Applications to mesh validity and bounds-preserving limiters

We introduce a novel method for bounding high-order multi-dimensional polynomials in finite element approximations. The method involves precomputing optimal piecewise-linear bounding boxes for polynomial basis functions, which can then be used to locally bound any combination of these basis functions. This approach can be applied to any element/basis type at any approximation order, can provide local (i.e., subcell) extremum bounds to a desired level of accuracy, and can be evaluated efficiently on-the-fly in simulations. Furthermore, we show that this approach generally yields more accurate bounds in comparison to traditional methods based on convex hull properties (e.g., Bernstein polynomials). The efficacy of this technique is shown in applications such as mesh validity checks and optimization for high-order curved meshes, where positivity of the element Jacobian determinant can be ensured throughout the entire element, and continuously bounds-preserving limiters for hyperbolic systems, which can enforce maximum principle bounds across the entire solution polynomial.

==> implementation.tex <==
%!TEX root = ./main.tex
\section{Implementation}\label{sec:implementation}


==> wip.tex <==
 %!TEX root = ./main.tex
\section{Preliminary Results}
\label{sec:wip}

% \begin{figure}[tbh!]
%   \begin{center}
%   $\begin{array}{c}
%   \includegraphics[width=0.9\linewidth]{figs/preliminary/untangling} \\
%   % \includegraphics[width=0.3\linewidth]{figures/2DSquareDiscOBB} \\
%   % \textrm{(d)} & \textrm{(e)} & \textrm{(f)}
%   \end{array}$
%   \end{center}
%   \vspace{-4mm}
%   \caption{Mesh untangled with barrier set as minimum bound}
% \label{fig_untangling_2D}
% \end{figure}


% \begin{figure}[tbh!]
%   \begin{center}
%   $\begin{array}{ccc}
%   \includegraphics[width=0.3\linewidth]{figs/preliminary/blade_orig_mesh} &
%   \includegraphics[width=0.3\linewidth]{figs/preliminary/blade_opt_no_bound_mesh} &
%   \includegraphics[width=0.3\linewidth]{figs/preliminary/blade_opt_bound_mesh} \\
%   \includegraphics[width=0.3\linewidth]{figs/preliminary/blade_orig_detJ} &
%   \includegraphics[width=0.3\linewidth]{figs/preliminary/blade_opt_no_bound_detJ} &
%   \includegraphics[width=0.3\linewidth]{figs/preliminary/blade_opt_bound_detJ} \\
%   % \includegraphics[width=0.3\linewidth]{figures/2DSquareDiscOBB} \\
%   % \textrm{(d)} & \textrm{(e)} & \textrm{(f)}
%   \end{array}$
%   \end{center}
%   \vspace{-4mm}
%   \caption{4th order mesh optimized without and with bounds on minimum determinant of the Jacobian.}
% \label{fig_blade}
% \end{figure}
